SANA: Efficient High-Resolution Image Synthesis with Linear Diffusion Transformers

We introduce Sana, a text-to-image framework that can efficiently generate images up to 4096$\times$4096 resolution. Sana can synthesize high-resolution, high-quality images with strong text-image alignment at a remarkably fast speed, deployable on laptop GPU. Core designs include: (1) Deep compression autoencoder: unlike traditional AEs, which compress images only 8$\times$, we trained an AE that can compress images 32$\times$, effectively reducing the number of latent tokens. (2) Linear DiT: we replace all vanilla attention in DiT with linear attention, which is more efficient at high resolutions without sacrificing quality. (3) Decoder-only text encoder: we replaced T5 with modern decoder-only small LLM as the text encoder and designed complex human instruction with in-context learning to enhance the image-text alignment. (4) Efficient training and sampling: we propose Flow-DPM-Solver to reduce sampling steps, with efficient caption labeling and selection to accelerate convergence. As a result, Sana-0.6B is very competitive with modern giant diffusion model (e.g. Flux-12B), being 20 times smaller and 100+ times faster in measured throughput. Moreover, Sana-0.6B can be deployed on a 16GB laptop GPU, taking less than 1 second to generate a 1024$\times$1024 resolution image. Sana enables content creation at low cost. Code and model will be publicly released.

==> figures_latext/ablation_y_norm.tex <==
\begin{wrapfigure}{r}{0.5\columnwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ablation_y_norm_scale_factor.jpg} 
    \caption{ablation y norm small scale factor (need show w/o norm will NaN). \ligeng{Either wrapfigure, subfigure} }
    \label{fig:ablation_y_norm_sf}
\end{wrapfigure}


==> figures_latext/flow_dpms_euler_sampler.tex <==
\begin{wrapfigure}{r}{0.5\columnwidth} 
    \centering
    \vspace{-6em}
    \includegraphics[width=0.9\linewidth]{figures/flow-sampler-ablation.pdf}
    \caption{\textbf{Impact of Sampling Steps on FID and CLIP Score}: A Comparison between Flow-DPM-Solver and Flow-Euler.
    }
    \label{fig:flow_sampler_ablation}
\end{wrapfigure}


==> tables/ablation_chi.tex <==
\begin{wraptable}{r}{0.5\columnwidth}
\centering
\caption{\textbf{Ablation study of whether using Complex Human Instruction (CHI).}}
\label{tab:ablation_chi}
\scalebox{0.8}{
\begin{tabular}{lll}
\toprule
\textbf{Prompt} & \textbf{Train Step} & \textbf{GenEval} \\
\midrule
User & \multirow{2}{*}{52k} & 45.5 \\
CHI + User & & 47.7~(+2.2) \\
\midrule
User & 140k & 52.8 \\
CHI + User & ~~+ 5k(ft) & 54.8~(+2.0) \\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{wraptable}


==> tables/ablation_dataset_clipscore.tex <==
\begin{table}[t]
\centering
\caption{\textbf{\footnotesize Performance of \model{} block design space.} We compare three image-text pair sampling strategies during training.}
\label{tab:dataset_clip_ablation}{
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Prompt Strategy & FID & CLIP \\
\midrule
Single & & \\
Multi-random & & \\
Multi-clipscore & & \\
\bottomrule
\end{tabular}
}
}
\end{table}


==> tables/ablation_y_norm.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation study of whether using text embedding normalization and the learnable scale factor initialization. (\enze{we have fig4 and no longer need it.})}}
\label{tab:results}{
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
\textbf{Text Embed Norm} & \textbf{Scale Factor} & \textbf{Train Step} & \textbf{FID} & \textbf{Clip Score} \\
\midrule
$\times$ & - & - & NaN & NaN \\
\multirow{2}{*}{$\checkmark$} & 1 & \multirow{2}{*}{16k} & 24.5 & 20.7 \\
 & 0.01 &  & 24.4 & 21.9 \\
\multirow{2}{*}{$\checkmark$} & 1 & \multirow{2}{*}{34k} & 14.6 & 23.5 \\
 & 0.01 &  & 13.1 & 24.3 \\
\multirow{2}{*}{$\checkmark$} & 1 & \multirow{2}{*}{52k} & 11.8 & 24.2 \\
 & 0.01 &  & 10.9 & 24.9 \\
\bottomrule
\end{tabular}
}
}
\end{table}


==> tables/speed_comparison.tex <==
\begin{table}[htbp]
\centering
\caption{Throughput and latency comparison at different resolutions. Test on one A100 GPU with FP16 precision.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{Methods} & \textbf{VAE} & \textbf{Resolution} & \textbf{Throughput} & \textbf{Latency} & \textbf{GPU (bs=1)} \\
\midrule
SD3 & F8C16P2 & 512/1K/2K/4K & 1.1/ 0.3/0.04/0.004 & 1.4/4.4/22/230 & 19G/22G/35G/70+G \\
FLUX-schnell-4step & F8C16P2 & 512/1K/2K/4K & 1.6/0.5/0.09/0.01 & 0.7/2.1/10.5/76 & 34G/37G/50G/70+G \\
FLUX-dev-50step & F8C16P2 & 512/1K/2K/4K & 0.3/0.1/0.01/0.001 & 4.5/13/66/1023 & 34G/37G/50G/70+G \\
PixArt-sigma-20step & F8C4P2 & 512/1K/2K/4K & 1.5/0.4/0.06/0.005 & 1.2/2.7/18.1/186 & 17G/18G/31G/70+G \\
HunyuanDlT-50step & F8C4P2 & 512/1K/2K/4K & 0.2/0.05/0.01/0.001 & 5.1/18.2/96/861 & 13G/13G/28G/70+G \\
\midrule
EDiT-0.6B-slim & F32C32P1 & 512/1K/2K/4K & 6.7/1.7/0.4/0.1 & 0.8/0.9/2.5/9.6 & 9G/11G/19G/45G \\
EDiT-1.6B & F32C32P1 & 512/1K/2K/4K & 3.8/1.0/0.25/0.06 & 0.6/1.2/4.1/15.9 & 13G/15G/24G/48G \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/train_schedule.tex <==
\begin{table}[th]
    \centering
    \caption{\textbf{\footnotesize Comparison of different training schedules. 120K steps, 256px.}}
    \label{tab:sampling_schedules}
    \resizebox{0.3\linewidth}{!}{ 
    \begin{tabular}{lccc}
        \toprule
        \textbf{Schedule} & \textbf{FID} & \textbf{CLIP} \\
        \midrule
        DDPM & 19.5 & 24.6 \\
        Flow Matching & 16.9 & 25.7 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-1em}
\end{table}


==> tables/vae_diffusion.tex <==
\begin{table}[th]
    \centering
    \caption{\textbf{\footnotesize Comparison of the impact of different VAE configurations on diffusion model performance.} 
    We explore factors such as latent size, VAE-diffusion compression ratios, and VAE channel variations. \ligeng{no longer need, remove}}
    \label{tab:vae_comparison}
    \resizebox{0.4\linewidth}{!}{ 
    \begin{tabular}{lccc}
        \toprule
        \textbf{VAE} & \textbf{rFID} & \textbf{FID} & \textbf{CLIP} \\
        \midrule
        F8C16P4+EDiT & 0.0884 & 21.9 & 24.1 \\
        F16C32P2+EDiT & 0.1618 & 13.7 & 24.6 \\
        F32C32P1+EDiT & 0.3421 & 7.3 & 25.8 \\
        \midrule
        F32C16P1+EDiT & 0.8649 & 7.2 & 25.8 \\
        F32C32P1+EDiT & 0.4608 & 7.3 & 25.8 \\
        F32C64P1+EDiT & 0.3141 & 10.6 & 25.3 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-1em}
\end{table}

